Gluing compact matrix quantum groups

We study glued tensor and free products of compact matrix quantum groups with cyclic groups -- so-called tensor and free complexifications. We characterize them by studying their representation categories and algebraic relations. In addition, we generalize the concepts of global colourization and alternating colourings from easy quantum groups to arbitrary compact matrix quantum groups. Those concepts are closely related to tensor and free complexification procedures. Finally, we also study a more general procedure of gluing and ungluing.

==> partmac.tex <==
%%Macro package for typeseting set partitions
%%Daniel Gromada 2019--2020
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%First, also as an example, we define shortcuts for some short partitions using word representation.

%%%Partitions with lower points only

%%k=1

\def\La{\LPartition{0.6:1}{}}

%%k=2

\def\Laa{\LPartition{}{0.6:1,2}}
\def\Lab{\LPartition{0.6:1,2}{}}

%k=3

\def\Laaa{\LPartition{}{0.6:1,2,3}}
\def\Laab{\LPartition{0.6:3}{0.6:1,2}}
\def\Laba{\LPartition{0.4:2}{0.8:1,3}}
\def\Labb{\LPartition{0.6:1}{0.6:2,3}}
\def\Labc{\LPartition{0.6:1,2,3}{}}

%k=4


\def\Laaaa{\LPartition{}{0.6:1,2,3,4}}
\def\Laaab{\LPartition{0.6:4}{0.6:1,2,3}}
\def\Laaba{\LPartition{0.4:3}{0.8:1,2,4}}
\def\Labaa{\LPartition{0.4:2}{0.8:1,3,4}}
\def\Labbb{\LPartition{0.6:1}{0.6:2,3,4}}
\def\Laabb{\LPartition{}{0.6:1,2;0.6:3,4}}
\def\Labba{\LPartition{}{0.8:1,4;0.4:2,3}}
\def\Labab{\LPartition{}{0.8:2,4;0.4:1,3}}
\def\Laabc{\LPartition{0.6:3,4}{0.6:1,2}}
\def\Labac{\LPartition{0.4:2,4}{0.8:1,3}}
\def\Labca{\LPartition{0.4:2,3}{0.8:1,4}}
\def\Labbc{\LPartition{0.6:1,4}{0.6:2,3}}
\def\Labcb{\LPartition{0.4:1,3}{0.8:2,4}}
\def\Labcc{\LPartition{0.6:1,2}{0.6:3,4}}
\def\Labcd{\LPartition{0.6:1,2,3,4}{}}

%%%Partitions with upper points only

%%k=1

\def\Ua{\UPartition{0.4:1}{}}

%%k=2

\def\Uaa{\UPartition{}{0.4:1,2}}
\def\Uab{\UPartition{0.4:1,2}{}}

%k=3

\def\Uaaa{\UPartition{}{0.5:1,2,3}}
\def\Uaab{\UPartition{0.4:3}{0.4:1,2}}
\def\Uaba{\UPartition{0.6:2}{0.2:1,3}}
\def\Uabb{\UPartition{0.4:1}{0.4:2,3}}
\def\Uabc{\UPartition{0.4:1,2,3}{}}

%k=4

\def\Uaaaa{\UPartition{}{0.4:1,2,3,4}}
\def\Uaaab{\UPartition{0.4:4}{0.4:1,2,3}}
\def\Uaaba{\UPartition{0.6:3}{0.2:1,2,4}}
\def\Uabaa{\UPartition{0.6:2}{0.2:1,3,4}}
\def\Uabbb{\UPartition{0.4:1}{0.4:2,3,4}}
\def\Uaabb{\UPartition{}{0.4:1,2;0.4:3,4}}
\def\Uabba{\UPartition{}{0.2:1,4;0.6:2,3}}
\def\Uabab{\UPartition{}{0.2:2,4;0.6:1,3}}
\def\Uaabc{\UPartition{0.4:3,4}{0.4:1,2}}
\def\Uabac{\UPartition{0.6:2,4}{0.2:1,3}}
\def\Uabca{\UPartition{0.6:2,3}{0.2:1,4}}
\def\Uabbc{\UPartition{0.4:1,4}{0.4:2,3}}
\def\Uabcb{\UPartition{0.6:1,3}{0.2:2,4}}
\def\Uabcc{\UPartition{0.4:1,2}{0.4:3,4}}
\def\Uabcd{\UPartition{0.4:1,2,3,4}{}}

%%%Partitions with same amount of upper and lower points

%%k=1, l=1

\def\Paa{\Partition{
\Pline (1,0) (1,1)
}}

\def\Pab{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
}}

%k=4

\def\Paaaa{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
\Pline (1.5,0.3) (1.5,0.7)
}}
\def\Paaab{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:2
\Pline (1,0) (1,0.7)
}}
\def\Paaba{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:1
\Pline (2,0) (2,0.7)
}}
\def\Pabaa{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1
\Pline (2,0.3) (2,1)
}}
\def\Pabbb{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:2
\Pline (1,0.3) (1,1)
}}
\def\Paabb{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabba{\Partition{
\Pline (1,0) (1,1)
\Pline (2,0) (2,1)
}}
\def\Pabab{\Partition{
\Pline (1,0) (2, 1)
\Pline (1,1) (2, 0)
}}
\def\Paabc{\Partition{
\Psingletons 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabcc{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}
\def\Pabac{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:1
\Pline (1,0) (2,1)
}}
\def\Pabcb{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:2
\Pline (2,0) (1,1)
}}
\def\Pabca{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
\Pline (2,0) (2,1)
}}
\def\Pabbc{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:2
\Pline (1,0) (1,1)
}}
\def\Pabcd{\Partition{
\Psingletons 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}

%k=6

\def\Pabcabc{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
}}
\def\Pabcabd{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:3
\Psingletons 1to0.7:1
}}
\def\Pabcadc{\Partition{
\Pline (1,0) (3, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:2
\Psingletons 1to0.8:2
}}
\def\Pabcdbc{\Partition{
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.3:1
\Psingletons 1to0.7:3
}}
\def\Pabcade{\Partition{
\Pline (1,0) (3, 1)
\Psingletons 0to0.2:2,3
\Psingletons 1to0.8:1,2
}}
\def\Pabcdec{\Partition{
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:1,2
\Psingletons 1to0.8:2,3
}}
\def\Pabcdbe{\Partition{
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:1,3
\Psingletons 1to0.7:1,3
}}
\def\Pabcdef{\Partition{
\Psingletons 0to0.3:1,2,3
\Psingletons 1to0.7:1,2,3
}}

\def\Paabaab{\Partition{
\Pblock 1to0.75:2,3
\Pblock 0to0.25:1,2
\Pline (1.5,0.25)(2.5,0.75)
\Pline (3,0)(1,1)
}}

%%%Some aliases

%\def\singleton{{\mathord{\uparrow}}}
%\def\upsingleton{{\mathord{\downarrow}}}
\def\singleton{\LPartition{\Ps1:1}{}}
\def\upsingleton{\UPartition{\Ps0:1}{}}
\let\pairpart=\Laa
\let\uppairpart=\Uaa
\let\fourpart=\Laaaa
\let\idpart=\Paa
\let\disconnecterpart=\Pab
\let\connecterpart=\Paaaa
\let\crosspart=\Pabab
\let\positionerpart=\Pabcb
\let\halflibpart=\Pabcabc


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%The macros

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}
\def\fihere#1\fi{\fi#1}

%definition of the \Partition command
\def\Partition#1{\def\Ptmp{#1}%
\futurelet\nextchar\PartitionB
}

\def\BigPartition#1{\def\Ptmp{#1}%
\futurelet\nextchar\BigPartitionB
}

\def\PartitionD{%
\thinspace\textchoice
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.175em}{0.55em}{0.7em}{\Ptmp}}
{\PartitionA{0.125em}{0.4em}{0.5em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}%
\thinspace%
}

\def\BigPartitionD{%
\thinspace\textchoice
{\PartitionA{1em}{0.9em}{2.5em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}
{\PartitionA{0.25em}{0.5em}{1em}{\Ptmp}}
{\PartitionA{0.20em}{0.4em}{0.8em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}%
\thinspace
}

\newcount\tmpx
\newcount\tmpy
\def\PartitionB{\if[\nextchar\let\next=\PartitionC\else\let\next=\PartitionD\fi\next}
\def\BigPartitionB{\if[\nextchar\let\next=\BigPartitionC\else\let\next=\BigPartitionD\fi\next}
\def\PartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\PartitionD}
\def\BigPartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\BigPartitionD}

\def\Ppointlist#1{\advance\tmpx by 1\if#1]\else
	\csname P#1\endcsname(\the\tmpx,\the\tmpy)
	\fihere\Ppointlist\fi}

\def\Pwidth{0.05}

\def\PartitionA#1#2#3#4{%
\pgfpicture
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Pwidth em}
#4
\endpgfpicture
}

%\Pline, \Psingletons, \Pblock, \Ptext,...

\def\Pline(#1,#2)#3(#4,#5){
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#5}}
\pgfusepath{stroke}
}

\def\Psingletons #1to#2:#3 {\PsingletonsA{#1}{#2}#3,,}
\def\PsingletonsA#1#2#3,{\ifx,#3,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfusepath{stroke}
\fihere\PsingletonsA{#1}{#2}\fi}

\def\Pblock #1to#2:#3 {\PblockA{#1}{#2}#3,,}
\def\PblockA#1#2#3,#4,{\ifx,#4,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#1}}
\pgfusepath{stroke}
\fihere\PblockA{#1}{#2}#4,\fi}

\def\Ptext(#1,#2)#3{%
\pgftext[at={\pgfpointxy{#1}{#2}}]{#3}
}

%\LPartition,\Upartition

\def\LPartition#1#2{\Partition{
\LPartitionB#2;;
\LPartitionA#1;;
}}

\def\LPartitionA#1;{\ifx;#1;\else
\Lsingletons #1 
\fihere\LPartitionA\fi}

\def\LPartitionB#1;{\ifx;#1;\else
\Pblock 0to#1 
\fihere\LPartitionB\fi}

\def\UPartition#1#2{\Partition{
\UPartitionB#2;;
\UPartitionA#1;;
}}

\def\UPartitionA#1;{\ifx;#1;\else
\Usingletons #1 
\fihere\UPartitionA\fi}

\def\UPartitionB#1;{\ifx;#1;\else
\Pblock 1to#1 
\fihere\UPartitionB\fi}

\def\Lsingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint0 #1#2 \else\Psingletons 0to#1#2 \fi
}
\def\Usingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint1 #1#2 \else\Psingletons 1to#1#2 \fi
}

%colors

\def\Pcolw{0.1}

\expandafter\def\csname P/\endcsname{\advance\tmpy by1 \tmpx=0}
\expandafter\def\csname P0\endcsname{}

\def\Pw (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
}

\def\Pb (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
}

\def\Ps#1(#2,#3){
	\pgfsetarrowsend{to}
	\pgfpathmoveto{\pgfpointxy{#2}{#3}}
	\pgfpathlineto{\pgfpointxy{#2}{#1}}
	\pgfusepath{stroke}
	\pgftransformreset
	\pgfsetarrowsend{}
}

\def\Pq (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\PQ (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\Lt (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\Ut (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\LT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}
\def\UT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}

\def\Ppoint #1 #2:#3 {\PpointA{#1}{#2}#3,,}
\def\PpointA#1#2#3,{\ifx,#3,\else #2(#3,#1)\fihere\PpointA{#1}{#2}\fi}

\def\coldefA #1 #2{\kern0.1ex\vcenter{\hbox{\def\Pcolw{#1}\pgfpicture#2(0,0)\endpgfpicture}}\kern0.1ex}

\def\coldef#1#2{\def#1{{\textchoice
{\coldefA 0.15 #2}{\coldefA 0.15 #2}{\coldefA 0.1 #2}{\coldefA 0.08 #2}{$\coldefA 0.15 #2$}}}}

\coldef\bcol\Pb
\coldef\wcol\Pw
\coldef\qcol\Pq
\coldef\Qcol\PQ
\coldef\tcol\Lt
\coldef\Tcol\LT

\def\idext{
	\Partition{
	\Ppoint0 \Lt:1
	\Ppoint1 \Ut:1
	}}
\def\positionerext{
	\Partition{
	\Ppoint0 \Lt:1
	\Ppoint1 \Ut:2
	\Pline(2,0)(1,1)
	}}
\def\globcolext{
	\Partition{
	\Ppoint0 \Lt:1
	\Ppoint1 \Ut:3
	\Pline(2,0)(1,1)
	\Pline(3,0)(2,1)
	}}

